A thin plate approximation for ocean wave interactions with an ice shelf

A variational principle is proposed to derive the governing equations for the problem of ocean wave interactions with a floating ice shelf, where the ice shelf is modelled by the full linear equations of elasticity and has an Archimedean draught. The variational principle is used to form a thin-plate approximation for the ice shelf, which includes water--ice coupling at the shelf front and extensional waves in the shelf, in contrast to the benchmark thin-plate approximation for ocean wave interactions with an ice shelf. The thin-plate approximation is combined with a single-mode approximation in the water, where the vertical motion is constrained to the eigenfunction that supports propagating waves. The new terms in the approximation are shown to have a major impact on predictions of ice shelf strains for wave periods in the swell regime.

==> Figs/Fig_strain_fields_0.tex <==
\input{./definitions-luke-fig}

%\def\showcomments{SHOWING COMMENTS}
%\def\shownewold{SHOWING NEW/OLD TEXT}
%\def\showdel{SHOWING DELETED TEXT}

\input{./colours-luke}
%\input{../JFM-21-1914.R1-production/annotations-luke}


%\def\figwidth{240pt}

\newlength{\figurewidth}
\newlength{\figwidth}
\newlength{\colsep}
\newlength{\figureheight}
\newlength{\myxunit}
\newlength{\rad}

\newlength{\textwidthGRL}
\setlength{\textwidthGRL}{\textwidth}

\begin{document}

\begin{my}

% Column width: \the\columnwidth;
% Text width: \the\textwidth;
% Text height: \the\textheight;
% Paperwidth: \the\paperwidth;
% Paperheight: \the\paperheight

\centering

\begin{tikzpicture}

 \newlength{\myfigwidth}
 
 \setlength{\figurewidth}{\textwidthGRL} 
 
 \node[inner sep=0pt,minimum width=\textwidthGRL,minimum height=0.64\textwidth,draw=none] (a) at (0,0) {};
 
% \setlength{\figurewidth}{0.45\textwidthGRL} 
% \setlength{\figureheight}{0.4\textwidthGRL} 
% \input{./Prods/Fig_RB_i} 
%
% \setlength{\figurewidth}{0.45\textwidthGRL}
% \setlength{\figureheight}{0.4\textwidthGRL} 
% \input{./Prods/Fig_RB_ii} 
 
 \setlength{\figurewidth}{\textwidthGRL}
 
 \input{./SubFig_strain_15s} 
 
 \input{./SubFig_strain_50s} 

 




 \end{tikzpicture}


\end{my}

\end{document}

==> Figs/SubFig_strain_15s.tex <==
% !TEX root = ./Fig_strain_fields.tex

\setlength{\myfigwidth}{\figurewidth}

 \node[inner sep=0pt,xshift=0pt,yshift=-5pt] (T15) at ($(a.north west)!0.5!(a.north east)$) [anchor=north] {\includegraphics[width=\myfigwidth,height=0.25\myfigwidth]{strain_fields_T15}}; 
 
\draw[black!85,line width=0.7pt] (T15.south west) -- ($(T15.south west)!0.975!(T15.south east)$) -- ($(T15.north west)!0.975!(T15.north east)$) -- (T15.north west) -- cycle;
 
\draw[black!85,line width=0.7pt] (T15.south east) -- ($(T15.south west)!0.985!(T15.south east)$) -- ($(T15.north west)!0.985!(T15.north east)$) -- (T15.north east) -- cycle;
  
\node[inner ysep=0pt,inner xsep=0pt,rotate=90,yshift=30pt,xshift=-0pt] at (T15.west) [anchor=center] {$z$\,[m]};

\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T15.south west)!0.9!(T15.north west)$) [anchor=east] {0};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T15.south west)!0.65!(T15.north west)$) [anchor=east] {$-50$}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T15.south west)!0.4!(T15.north west)$) [anchor=east] {$-100$}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T15.south west)!0.15!(T15.north west)$) [anchor=east] {$-150$}; 

\node[inner ysep=0pt,inner xsep=0pt,rotate=-90,yshift=20pt,xshift=-0pt] at (T15.east) [anchor=center] {$\vert{}\hat{\varepsilon}_{11}\vert$ $\times{}10^{7}$};

\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T15.south east)!0.02!(T15.north east)$) [anchor=east] {0};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T15.south east)!0.22!(T15.north east)$) [anchor=east] {1}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T15.south east)!0.43!(T15.north east)$) [anchor=east] {2};  
 \node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T15.south east)!0.64!(T15.north east)$) [anchor=east] {3};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=-0pt,rotate=0] at ($(T15.south east)!0.85!(T15.north east)$) [anchor=east] {4};  

\node[align=center,anchor=north west,white] at (T15.north west) {(a)};


==> Figs/SubFig_strain_50s.tex <==
% !TEX root = ./Fig_strain_fields.tex

\setlength{\myfigwidth}{\figurewidth}

 \node[inner sep=0pt,xshift=0pt,yshift=-10pt] (T50) at (T15.south) [anchor=north] {\includegraphics[width=\myfigwidth,height=0.25\myfigwidth]{strain_fields_T50}}; 
 
\node[inner ysep=0pt,inner xsep=0pt,rotate=0,xshift=0pt,yshift=-15pt] at (T50.south) [anchor=north] {$x$\,[km]};

\draw[black!85,line width=0.7pt] (T50.south west) -- ($(T50.south west)!0.975!(T50.south east)$) -- ($(T50.north west)!0.975!(T50.north east)$) -- (T50.north west) -- cycle;

\draw[black!85,line width=0.7pt] (T50.south east) -- ($(T50.south west)!0.985!(T50.south east)$) -- ($(T50.north west)!0.985!(T50.north east)$) -- (T50.north east) -- cycle;

\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.0!(T50.south east)$) [anchor=north] {0}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.195!(T50.south east)$) [anchor=north] {1}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.39!(T50.south east)$) [anchor=north] {2}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.585!(T50.south east)$) [anchor=north] {3}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.78!(T50.south east)$) [anchor=north] {4}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=0pt,yshift=-2pt,rotate=0] at ($(T50.south west)!0.975!(T50.south east)$) [anchor=north] {5};

\node[inner ysep=0pt,inner xsep=0pt,rotate=90,yshift=30pt,xshift=-0pt] at (T50.west) [anchor=center] {$z$\,[m]};

\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T50.south west)!0.9!(T50.north west)$) [anchor=east] {0};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T50.south west)!0.65!(T50.north west)$) [anchor=east] {$-50$}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T50.south west)!0.4!(T50.north west)$) [anchor=east] {$-100$}; 
\node[inner ysep=0pt,inner xsep=0pt,xshift=-2pt,yshift=-0pt,rotate=0] at ($(T50.south west)!0.15!(T50.north west)$) [anchor=east] {$-150$}; 

\node[inner ysep=0pt,inner xsep=0pt,rotate=-90,yshift=20pt,xshift=-0pt] at (T50.east) [anchor=center] {$\vert{}\hat{\varepsilon}_{11}\vert$ $\times{}10^{5}$};

\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T50.south east)!0.02!(T50.north east)$) [anchor=east] {0};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T50.south east)!0.25!(T50.north east)$) [anchor=east] {2};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T50.south east)!0.48!(T50.north east)$) [anchor=east] {4};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=0pt,rotate=0] at ($(T50.south east)!0.71!(T50.north east)$) [anchor=east] {6};  
\node[inner ysep=0pt,inner xsep=0pt,xshift=8pt,yshift=-0pt,rotate=0] at ($(T50.south east)!0.95!(T50.north east)$) [anchor=east] {8};  

\node[align=center,anchor=north west,white] at (T50.north west) {(b)};



==> Figs/colours-luke.tex <==
\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0,0.55,0}
\definecolor{midgreen}{rgb}{0,0.8,0.2}
\definecolor{magenta}{rgb}{1,0,1}
\definecolor{purple}{rgb}{0.5,0,0.5}
\definecolor{darkorange}{rgb}{1,0.55,0}
\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{olive}{rgb}{0.5,0.5,0}
\definecolor{midgrey}{rgb}{0.5,0.5,0.5}
\definecolor{lightgrey}{rgb}{0.75,0.75,0.75}
\definecolor{matlabblue}{rgb}{0,0.447,0.741}
\definecolor{matlabred}{rgb}{0.85,0.325,0.098}
\definecolor{lightblue}{rgb}{0,0.5,1}
\definecolor{lightcyan}{rgb}{0,0.8,0.8}
\definecolor{darkgrey}{rgb}{0.25,0.25,0.25}
\definecolor{teal}{rgb}{0,0.5,0.5}
\definecolor{navy}{rgb}{0,0,0.5}
\definecolor{goldenrod}{rgb}{0.85,0.6,0.1}

==> boxes-luke.tex <==
%% BOXES

\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
\definecolor{mycolor}{rgb}{0.122, 0.435, 0.698}% Rule colour
\makeatletter
\newcommand{\tbox}[5]{
\setbox0=\hbox{#1}%
\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
\begin{tcolorbox}[colback=#3,colframe=#4,
      boxrule=#5,arc=4pt,
      left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt,
      width=#2]   %\@tempdima]
    #1
\end{tcolorbox}}
\makeatother

\NewDocumentCommand\mybox{om}{%
\IfNoValueTF{#1}{
\tbox{#2}{\textwidth}{white}{mycolor}{2pt}
}{
\tbox{#2}{#1}{white}{mycolor}{2pt}
}}

%\NewDocumentCommand\mytitlebox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{gray!30}{mycolor}{0pt}
%}{
%\tbox{#2}{#1}{gray!30}{mycolor}{0pt}
%}}
%
%\NewDocumentCommand\myparbox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{blue!10}{white}{0pt}
%}{
%\tbox{#2}{#1}{blue!10!white!90}{white}{0pt}
%}}
